Can MLLMs Reason in Multimodality? EMMA: An Enhanced MultiModal ReAsoning Benchmark

The ability to organically reason over and with both text and images is a pillar of human intelligence, yet the ability of Multimodal Large Language Models (MLLMs) to perform such multimodal reasoning remains under-explored. Existing benchmarks often emphasize text-dominant reasoning or rely on shallow visual cues, failing to adequately assess integrated visual and textual reasoning. We introduce EMMA (Enhanced MultiModal reAsoning), a benchmark targeting organic multimodal reasoning across mathematics, physics, chemistry, and coding. EMMA tasks demand advanced cross-modal reasoning that cannot be addressed by reasoning independently in each modality, offering an enhanced test suite for MLLMs' reasoning capabilities. Our evaluation of state-of-the-art MLLMs on EMMA reveals significant limitations in handling complex multimodal and multi-step reasoning tasks, even with advanced techniques like Chain-of-Thought prompting and test-time compute scaling underperforming. These findings underscore the need for improved multimodal architectures and training paradigms to close the gap between human and model reasoning in multimodality.

==> sec/4.3.2_Qwen-RM.tex <==
\begin{table*}[t]
    \centering
    \small
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{ccccccc}
    \toprule
    \textbf{Model} & \textbf{Method} & \textbf{N=1} & \textbf{N=2} & \textbf{N=4} & \textbf{N=8} & \textbf{N=16} \\
    \midrule
    \multirow[c]{3}{*}{GPT-4o} & BoN w. Self-RM & \multirow{3}{*}{27.00} & 29.00 & 27.00 & 25.00 & $-$ \\
     & BoN w. Gemini 2.0 Flash Thinking as RM &  & \second{30.00} & 28.00 & \best{31.00} & $-$ \\
     & BoN w. Qwen2.5-Math-RM-72B as RM &  & 26.00 & 24.00 & 25.00 & 29.00  \\
    \midrule
    \multirow[c]{3}{*}{Gemini 2.0 Flash} & BoN w. Self-RM & \multirow{3}{*}{24.00} & \best{33.00} & 24.00 & 27.00 & $-$ \\
     & BoN w. Gemini 2.0 Flash Thinking as RM &  & \best{33.00} & 24.00 & 25.00 & $-$ \\
     & BoN w. Qwen2.5-Math-RM-72B as RM &  & 27.00 & 28.00 & 23.00 & 23.00  \\
    \midrule
    Gemini 2.0 Flash Thinking & $-$ & \best{35.00} & $-$ & $-$ & $-$ & $-$  \\
    \midrule
    o1 & $-$ & \best{41.00} & $-$ & $-$ & $-$ & $-$ \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Test-time scaling results on the math portion of EMMA-mini using Qwen2.5-Math-RM-72B as the RM. Since the RM does not take images as input, we provide captions of images in the problems to it. Benefits of scaling plateau quickly start to plateau. 
    \linjie{we shall also add the result of BoN with self-RM and strong-RM, to highlight whether a text-only specialized Math RM is better or worse than general purpose RM. and discuss how far away open-source is from the best closed-source models as RM.}
    \linjie{we may also need some explanation why N=2 -> N=4 dropped by 4 points for gemini flash. but not for 4o. looks like we need an example of how RM evaluates the predictions, may show one good example of the same question with two model predictions + scores from Qwen2.5-Math-RM, and the tournament output from Gemini thinking. And another bad example.}
    } 
    \label{tab:math scaling}
\end{table*}

\paragraph{Best-of-N With a Specialized Math Reward Model} \linjie{move to appendix, and mention we have additional experiments  + we do not have open-source specialized multimodal reward models in Best-of-N above}
While we also want to evaluate specialized reward models, they are currently only available for math. Qwen2.5-Math-RM-72B~\cite{yang2024qwen2} is one such specialized LLM for evaluating the quality of responses to math problems. For the math portion of EMMA-mini, we first generate 16 responses using each of GPT-4o and Gemini~2.0~Flash. We then score each response using Qwen2.5-Math-RM-72B and select the highest-scoring answer. As in previous experiments, we test with \textit{N} values of 4, 8, and 16. Since Qwen2.5-Math-RM-72B is not multimodal, we supply GPT-4o-generated captions for all images in the questions to enable evaluation. %\linjie{Need to mention where did the caption come. } 


Table~\ref{tab:math scaling} focuses specifically on scaling for the math portion of EMMA-mini with a specialized RM. 
\linjie{also need more discussions about table 4, the discussion below is too high-level, nice to use as the concluding sentence.}

on emma-mini:

on math: closed source stronger than open source, but note that qwen2 used here is not multimodal; similar to above, scaling beyond 8 does not help; similar to above, thinking as rm gives the best performance; perhaps limited by candidate response generator performance, 

==> sec/storage.tex <==
\begin{enumerate}
    \item \textbf{Velocity at $t_A$ ($\vec{v}_A$):} 
    \[
    \vec{v}_A \text{ points upward ($+y$) and to the right ($+x$).}
    \]

    \item \textbf{Velocity at $t_B$ ($\vec{v}_B$):}
    \[
    \vec{v}_B \text{ points upward ($+y$) and to the left ($-x$).}
    \]

    \item \textbf{Acceleration:}
    \[
    \vec{a} = \frac{\Delta \vec{v}}{\Delta t} = \frac{\vec{v}_B - \vec{v}_A}{\Delta t} = \frac{\vec{v}_B + (-\vec{v}_A)}{\Delta t}
    \]
    Here, $-\vec{v}_A$ points downward ($-y$) and to the left ($-x$).

    \item \textbf{Net Direction:}
    \begin{itemize}
        \item Horizontal components ($+x$, $-x$) partially cancel.
        \item Vertical components ($+y$, $-y$) combine, resulting in a downward ($-y$) vector.
    \end{itemize}
    \item \textbf{Conclusion}
    \begin{itemize}
    \item The net acceleration points downward ($-y$), corresponding to option \textbf{b}.
    \end{itemize}






\end{enumerate}




Steps:
\begin{enumerate}
    \item Compute the change in velocity:
    \[
    \Delta \vec{v} = \vec{v}_f - \vec{v}_i.
    \]
    \item Represent $\Delta \vec{v}$ graphically by:
    \[
    \vec{B} + (-\vec{A}),
    \]
    where $-\vec{A}$ is the opposite of $\vec{A}$.
    \item Place the $\vec{B}$ vector "tip-to-tail" with the $-\vec{A}$ vector. The resulting direction of $\Delta \vec{v}$ (and therefore $\vec{a}$) points to the left.
\end{enumerate}
